Unsupervised Word Segmentation from Discrete Speech Units in Low-Resource Settings

Documenting languages helps to prevent the extinction of endangered dialects, many of which are otherwise expected to disappear by the end of the century. When documenting oral languages, unsupervised word segmentation (UWS) from speech is a useful, yet challenging, task. It consists in producing time-stamps for slicing utterances into smaller segments corresponding to words, being performed from phonetic transcriptions, or in the absence of these, from the output of unsupervised speech discretization models. These discretization models are trained using raw speech only, producing discrete speech units that can be applied for downstream (text-based) tasks. In this paper we compare five of these models: three Bayesian and two neural approaches, with regards to the exploitability of the produced units for UWS. For the UWS task, we experiment with two models, using as our target language the Mboshi (Bantu C25), an unwritten language from Congo-Brazzaville. Additionally, we report results for Finnish, Hungarian, Romanian and Russian in equally low-resource settings, using only 4 hours of speech. Our results suggest that neural models for speech discretization are difficult to exploit in our setting, and that it might be necessary to adapt them to limit sequence length. We obtain our best UWS results by using Bayesian models that produce high quality, yet compressed, discrete representations of the input speech signal.

==> figures/segmentation_pic.tex <==
% \begin{figure}
% \centering
% \begin{subfigure}[t]
%     \includegraphics{tables/vq_vae_seg.png}
%     \caption{VQ-VAE}
%     \label{fig:vq_vae_seg}
% \end{subfigure}
% \begin{subfigure}
%     \includegraphics{tables/hmm_seg.png}
%     \caption{HMM}
%     \label{fig:hmm_seg}
% \end{subfigure}
% \begin{subfigure}
%     \includegraphics{tables/shmm_seg.png}
%     \caption{SHMM}
%     \label{fig:shmm_seg}
% \end{subfigure}
% \begin{subfigure}
%     \includegraphics{tables/hshmm_seg.png}
%     \caption{HSHMM}
%     \label{fig:hshmm_seg}
% \end{subfigure}
% \end{figure}
\begin{figure*}
     \centering
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/vq_vae_seg_same.png}
         \caption{VQ-VAE}
         \label{fig:vqvae_seg}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/hmm_seg_same.png}
         \caption{HMM}
         \label{fig:hmm_seg}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/shmm_seg_same.png}
         \caption{SHMM}
         \label{fig:shmm_seg}
     \end{subfigure}
     \begin{subfigure}[b]{\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/hshmm_seg_same.png}
         \caption{H-SHMM}
         \label{fig:hshmm_seg}
     \end{subfigure}
    \caption{Unit segmentation for the same Mboshi sentence by each AUD system. The black lines denote the true boundaries, %between the actual phones 
    while the dashed white lines denote the unit boundaries %of the units 
    discovered by each AUD system. The symbols at the bottom of each image correspond to the reference, while those at the top correspond to the predicted units.}
    \label{fig:segmentation}
\end{figure*}


% \begin{figure}
%      \centering
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{tables/vq_vae_seg2.png}
%          \caption{VQ-VAE}
%          \label{fig:vqvae_seg2}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{tables/hmm_seg2.png}
%          \caption{HMM}
%          \label{fig:hmm_seg2}
%      \end{subfigure}
%      \hfill
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{tables/shmm_seg2.png}
%          \caption{SHMM}
%          \label{fig:shmm_seg2}
%      \end{subfigure}
%      \begin{subfigure}[b]{\textwidth}
%          \centering
%          \includegraphics[width=\textwidth]{tables/hshmm_seg2.png}
%          \caption{H-SHMM}
%          \label{fig:hshmm_seg2}
%      \end{subfigure}
%     \caption{Segmentations}
%     \label{fig:seg}
% \end{figure}

==> tables/seg_stats.tex <==
\begin{table}[t]
    \caption{Segmentation statistics for the Mboshi dataset using the neural UWS model.}
\centering
\resizebox{7.3cm}{!}{
\begin{tabular}{lcccc}
\toprule
\multicolumn{1}{l}{} & \# Types & \# Tokens & \begin{tabular}[c]{@{}c@{}}Avg token \\ length\end{tabular} & \begin{tabular}[c]{@{}c@{}}Avg \# token\\ per sentence\end{tabular} \\\midrule
\textbf{VQ-VAE - SIL}      & 21,708   & 38,431    & 5.8                                                         & 7.5                                                                 \\
\textbf{HMM - SIL}         & 15,285   & 29,415    & 3.7                                                         & 5.7                                                                 \\
\textbf{SHMM - SIL}        & 16,212   & 26,488    & 3.9                                                         & 5.2                                                                 \\
\textbf{H-SHMM - SIL}       & 14,738   & 27,413    & 3.6                                                         & 5.3                                                                 \\
\textbf{Reference}   & 5,162    & 42,715    & 3.2                                                         & 5.8                                     \\\bottomrule                           
\end{tabular}}

    \label{tab:segstats}
\end{table}
